Competitive Parallelism: Getting Your Priorities Right

Multi-threaded programs have traditionally fallen into one of two domains: cooperative and competitive. These two domains have traditionally remained mostly disjoint, with cooperative threading used for increasing throughput in compute-intensive applications such as scientific workloads and cooperative threading used for increasing responsiveness in interactive applications such as GUIs and games. As multicore hardware becomes increasingly mainstream, there is a need for bridging these two disjoint worlds, because many applications mix interaction and computation and would benefit from both cooperative and competitive threading. In this paper, we present techniques for programming and reasoning about parallel interactive applications that can use both cooperative and competitive threading. Our techniques enable the programmer to write rich parallel interactive programs by creating and synchronizing with threads as needed, and by assigning threads user-defined and partially ordered priorities. To ensure important responsiveness properties, we present a modal type system analogous to S4 modal logic that precludes low-priority threads from delaying high-priority threads, thereby statically preventing a crucial set of priority-inversion bugs. We then present a cost model that allows reasoning about responsiveness and completion time of well-typed programs. The cost model extends the traditional work-span model for cooperative threading to account for competitive scheduling decisions needed to ensure responsiveness. Finally, we show that our proposed techniques are realistic by implementing them as an extension to the Standard ML language.

==> elab.tex <==
\section{Elaboration of {\langname} to {\calcname}}\label{sec:elab}

In this section, we define an elaboration from {\langname} to {\calcname}. This
can be seen as giving a formal semantics to {\langname} programs by placing
them in correspondence with {\calcname} programs. We begin by formally defining
the syntax of {\langname}, in Figure~\ref{fig:elab-syn}. We use the
metavariables~$\eexp$ and~$\ecmd$ (and variants) to refer to {\langname}
expressions and commands, respectively, in order to distinguish them from their
{\calcname} counterparts. We also add syntactic classes for
instructions~$\inst$, priority annotations~$\priocons$, declarations~$\decl$,
toplevel declarations~$\tdecl$ and programs~$\prog$.
Expressions are more or less the same as in
{\calcname}, with the addition of let bindings, which introduce zero or more
declarations into the scope of an expression (the notation~$\multi{\decl}$
stands for a list of declarations). The command layer of {\langname} is split
into two syntactic classes: commands and instructions, where a command is a
sequence of instructions, each binding its return value, ending in a return.
Instructions now include~\kwdo{e}, which runs an encapsulated command
(expressible in {\langname} as $\kwbind{e}{x}{\kwret{x}}$).
Declarations~$\decl$, which may be included in let bindings, introduce
expressions, functions (which bind one or more variables, indicated by the
notation~$\multip{x}$), or priority-level functions (which bind one or more
priority variables and one or more expression variables). All of these
declarations can appear at the top level, as can priority and order
declarations. These are the separate class of toplevel declarations.
Finally, a program is zero or more toplevel declarations followed by a command
to run as the ``main'' thread.

For simplicity of the formal definition of elaboration, a number of features
of {\langname} are omitted from the formalism. For example, we include natural
numbers and unit as the only base type, while {\langname} has integers,
booleans, strings, etc. We also omit many useful features of a language such
as algebraic datatypes, mutually recursive functions and exceptions.
These are present in our
implementation (although we have not implemented mutually recursive
priority-level functions).
The elaboration of these features is standard (e.g.~\citep{HarperSt96}).

\input{fig-elab}

The main work of elaboration is converting declarations in {\langname} to
(possibly recursive) functions (both expression- and priority-level)
in {\calcname}, converting let bindings to function application, and hoisting
priority and order declarations out of the code so that they may be presented
as a pre-defined partially-ordered set, as required by the {\calcname}
semantics. The overall goal of elaboration then is to convert a
{\langname} program~$\prog$ into a {\calcname} command~$\cmd$ together with a
partial order~$\worlds$ of priorities.
This proceeds in a number of mutually recursive stages, with one elaboration
judgment for each syntactic class of {\langname}.

Each judgment, except the
one for programs, is annotated with the type of the {\calcname} expression or
command that is produced by elaboration. In this sense, elaboration is typed.
We do not explicitly define a static semantics for {\langname}. Instead, the
static semantics is given by elaboration itself. If a {\langname} program
evaluates to a {\calcname} command, that command will be well-typed at
a distinguished priority~\code{bot} (abstractly notated~$\bot$) with the
type given in the elaboration judgment (Theorem~\ref{thm:elab-corr}). If the
elaboration rules do not allow a valid elaboration to be derived for a
{\langname} program, then we will reject that program as ill-typed.

The elaboration judgments are:
\begin{itemize}
\item $\elabexp{\ctx}{\eexp}{e}{\tau}$ converts a {\langname} expression to
  a {\calcname} expression.
\item $\elabinst{\ctx}{\inst}{e}{\tau}{\prio}$ converts a
  {\langname} instruction to a {\calcname} command.
  These will be sequenced together using the bind operator of {\calcname}.
\item $\elabcmd{\ctx}{\ecmd}{\cmd}{\tau}{\prio}$ converts a {\langname}
  command to a {\calcname} command.
\item $\elabdecl{\ctx}{\decl}{x}{e}{\tau}$ converts a {\langname} declaration
  to the variable it binds together with the {\calcname} expression bound to
  it.
\item $\elabprog{\worlds}{\ctx}{\prog}{\cmd}{\worlds'}{\ctx'}$
  converts a {\langname} program to a {\calcname} command, together with a
  partially ordered set of priorities. The existing partial order~$\worlds$ is
  extended by~$\worlds'$.
\end{itemize}

The elaboration rules for expressions are defined in Figure~\ref{fig:elab-exp}.
\ifproofs
These rules are mostly straightforward, and closely follow the typing rules.
\else
These rules are mostly straightforward, and closely follow the typing rules,
so we show only a few rules as examples.
\fi
The rules of interest are those for let bindings. For each declaration in
sequence, the declaration is elaborated into a pair~$(x, e')$. The
body of the let binding (together with the elaboration of the remaining
bindings) is wrapped in a $\lambda$-abstraction binding the variable~$x$,
which is applied to~$e'$.%\footnote{The empty let binding with no declarations,
%  in addition to being a useful base case for these rules, is valid, if
%  rarely used, Standard ML syntax.}

The elaboration rules for instructions and commands are defined in
Figure~\ref{fig:elab-thread}. The elaboration rule for~\kw{do} instructions
evaluates the expression, checks that it has the type of an encapsulated
command, and elaborates it to a command that uses the bind operation of
{\calcname} to bind the command's return value to a fresh variable.
Other instructions elaborate to the
corresponding command (with any sub-components recursively elaborated).
This uniformly produces a command for each
instruction, which can be sequenced together using binding in the first
command elaboration rule. The second command elaboration rule, for~\code{ret},
simply elaborates the final instruction into a command.
The~$\cmd_1; \cmd_2$ form of sequencing we used in Section~\ref{sec:overview},
which does not bind the return value of~$\cmd_1$, can easily be desugared
to~$\kwbind{\cmd_1}{x}{\cmd_2}$, where~$x$ does not appear free in~$\cmd_2$.
To keep the formalism simple, this syntactic sugar is not included in the rules.

The elaboration rules for declarations and programs appear in
Figure~\ref{fig:elab-prog}. The rule for~\code{val} declarations simply
elaborates the expression and returns a pair of the bound variable and
elaborated expression. Function declarations (both expression-level and
priority-level) are recursive, and so elaborating them involves finding a fixed
point. The elaboration of priority-monomorphic~\code{fun} declarations
elaborates the body in
a context that includes all of the arguments, as well as the function itself.
This is then placed inside~$n$ nested $\lambda$-abstractions to bind the
required arguments. Finally, this expression is nested inside a fixed-point
operator to introduce the recursive binding of the function name.
Something similar occurs for priority-polymorphic~\code{fun} declarations.
The body is nested
inside~$m$ $\lambda$-abstractions to introduce the expression variables,
followed by $n$ priority-level abstractions to introduce the priority variables.
Finally, this whole expression is wrapped in a fixed-point operator.

The last elaboration judgment covers both toplevel declarations and programs,
and produces a command corresponding to the entire {\langname} program.
The first three rules for this judgment elaborate each form of toplevel
declaration followed by the remainder of the program, and the final rule
evaluates the ``main'' command that terminates the program.
Priority and order declarations are erased from the program; their elaboration
is simply the elaboration of the remainder of the program. However, the
priorities and ordering relations introduced by these declarations are collected
into the partial order that will be returned at the end of elaboration. Each time a new
ordering constraint~$\plt{\prioc_1}{\prioc_2}$ is introduced, we check that
$\nple{\prioc_2}{\prioc_1}$. This premise checks that the new constraint will
not induce a cycle in the priority relation and ensure that the generated
relation is a valid partial order. Ordinary declarations (\code{val} and
\code{fun}) at
the top level are elaborated using the declaration elaboration rules. Before
elaborating these declarations, the current set of worlds and ordering
constraints is loaded into the context as follows, assuming~$\worlds$ contains
priorities~$\{\prioc_1, \dots, \prioc_n\}$ with ordering
relation~$\{(\prioc_1, \prioc_1'), \dots, (\prioc_m, \prioc_m')\}$.
\[
\ctxify{\worlds} = \prioc_1 \isprio, \dots, \prioc_n \isprio,
\ple{\bot}{\prioc_1}, \dots, \ple{\bot}{\prioc_n},
\ple{\prioc_1}{\prioc_1'}, \dots, \ple{\prioc_m}{\prioc_m'}
  \]
The
elaborated expression is wrapped in a command and then introduced using binding.
%Finally, the main command is elaborated at priority~$\bot$ and returned.
Loading the bindings into the context types the same constraints,
expressions and commands as
providing the partial order as a parameter to the judgment.

\begin{lem}\label{lem:ctxify}
  \begin{enumerate}
  \item
  If $\meetc[]{\ctxify{\worlds}, \ctx}{\cons}$, then
  $\meetc[\worlds]{\ctx}{\cons}$.
  \item
  If $\etyped[]{\esig}{\ctxify{\worlds}, \ctx}{e}{\tau}$, then
  $\etyped[\worlds]{\esig}{\ctx}{e}{\tau}$.
  \item
  If $\cmdtyped[]{\esig}{\ctxify{\worlds}, \ctx}{\cmd}{\tau}{\prio}$, then
  $\cmdtyped[\worlds]{\esig}{\ctx}{\cmd}{\tau}{\prio}$.
  \end{enumerate}
\end{lem}
\begin{proof}
  We show part (1) by induction on the derivation of
  $\meetc[]{\ctxify{\worlds}, \ctx}{\cons}$. The interesting case
  is~$\meetc[]{\ctx', \ple{\prioc_1}{\prioc_2}, \ctx}{\cons}$,
  where~$\plt{\prioc_1}{\prioc_2} \in \worlds$. Apply rule~\rulename{assume}.
  Parts (2) and (3) are then straightforward inductions, the only interesting
  cases of which are applications of (1).
\end{proof}

Theorem~\ref{thm:elab-corr} shows that elaboration is type-correct in that
elaboration will produce a well-typed {\calcname} program. The theorem has a
conjunct for each elaboration judgment.

\begin{thm}[Correctness of elaboration]\label{thm:elab-corr}
\begin{enumerate}
\item If $\elabexp{\ctx}{\eexp}{e}{\tau}$, then $\etyped[]{\esig}{\ctx}{e}{\tau}$.
\item If $\elabinst{\ctx}{\inst}{\cmd}{\tau}{\prio}$, then
  $\cmdtyped[]{\esig}{\ctx}{\cmd}{\tau}{\prio}$.
\item If $\elabcmd{\ctx}{\ecmd}{\cmd}{\tau}{\prio}$, then
  $\cmdtyped[]{\esig}{\ctx}{\cmd}{\tau}{\prio}$.
\item If $\elabdecl{\ctx}{\decl}{x}{e}{\tau}$, then
  $\etyped[]{\esig}{\ctx}{e}{\tau}$.
\item If $\elabprog{\worlds}{\ctx}{\prog}{\cmd}{\worlds'}{\ctx'}$,
  then  $\cmdtyped[\worlds \cup \worlds']{\esig}{\ctx}
  {\cmd}{\tau}{\bprio}$.
\end{enumerate}
\end{thm}

\begin{proof}
\begin{enumerate}
\item By induction on the derivation of $\elabexp{\ctx}{\eexp}{e}{\tau}$.
%%   \begin{itemize}
%%   \item Apply rule \rulename{\kwunit I}.
%%   \item Apply rule \rulename{\kwnat I}.
%%   \item By inversion, $\elabexp{\ctx}{\eexp}{e}{\kwnat}$ and
%%   $\elabexp{\ctx}{\eexp_1}{e_1}{\tau}$ and
%%   $\elabexp{\ctx, \hastype{x}{\kwnat}}{\eexp_2}{e_2}{\tau}$.
%%   By induction, $\etyped[]{\esig}{\ctx}{e}{\kwnat}$ and
%%   $\etyped[]{\esig}{\ctx}{e_1}{\tau}$ and
%%   $\etyped[]{\esig}{\ctx, \hastype{x}{\kwnat}}{e_2}{\tau}$.
%%   Apply rule \rulename{\kwnat E}.
%%   \item
%%   \item
%%   \item
%%   \item
%%   \item
%%   \item
%%   \item
%%   \item
%%   \item
%%   \item
%%   \item
%%   \item By inversion, $\elabexp{\ctx}{\eexp}{e}{\tau}$.
%%   By induction, $\etyped[]{\esig}{\ctx}{e}{\tau}$.
%%   \item By inversion, $\elabdecl{\ctx}{\decl}{x}{e'}{\tau'}$ and
%%   $\elabexp{\ctx, \hastype{x}{\tau'}}{\kwlet{\multi{\decl}}{\eexp}}{e}{\tau}$.
%%   By induction, $\etyped[]{\esig}{\ctx}{e'}{\tau'}$ and
%%   $\elabexp{\esig}{\ctx, \hastype{x}{\tau'}}{e}{\tau}$.
%%   Apply rules \rulename{\arrsym I} and \rulename{\arrsym E}.
%% \item
%% \item By inversion, $\elabexp{\ctx}{\eexp}{e}{\kwforall{\vprio}{\cons}{\tau}}$
%%   and $\meetc[]{\ctx}{[\prio'/\vprio]\cons}$.
%%   By induction, $\etyped[]{\esig}{\ctx}{e}{\kwforall{\vprio}{\cons}{\tau}}$.
%%   Apply rule \rulename{\fasym E}.
%%   \end{itemize}
\item By induction on the derivation of $\elabinst{\ctx}{\inst}{\cmd}{\tau}{\prio}$.
  \ifproofs
  \begin{itemize}
  \item By inversion, $\elabexp{\ctx}{\eexp}{e}{\kwcmdt{\tau}{\prio'}}$.
    By induction, $\etyped[]{\esig}{\ctx}{e}{\kwcmdt{\tau}{\prio'}}$.
    Apply rules \rulename{\cmdsym I}, \rulename{Bind} and \rulename{Var}.
  \item By inversion, $\elabexp{\ctx}{\eexp}{e}{\kwat{\tau}{\prio'}}$.
  By induction, $\etyped[]{\esig}{\ctx}{e}{\kwat{\tau}{\prio'}}$.
  Apply rule \rulename{Sync}.
  \item By inversion, $\elabcmd{\ctx}{\ecmd}{\cmd}{\tau}{\prio'}$.
  By induction, $\cmdtyped[]{\esig}{\ctx}{\cmd}{\tau}{\prio'}$.
  Apply rule \rulename{Spawn}.
  \item By inversion, $\elabexp{\ctx}{\eexp}{e}{\tau}$.
  By induction, $\etyped[]{\esig}{\ctx}{e}{\tau}$. Apply rule \rulename{Ret}.

  \end{itemize}
  \fi
\item By induction on the derivation of $\elabcmd{\ctx}{\ecmd}{\cmd}{\tau}{\prio}$.
  \ifproofs
  \begin{itemize}
  \item By inversion, $\elabinst{\ctx}{\inst}{\cmd}{\tau}{\prio}$
  and $\elabcmd{\ctx, \hastype{x}{\tau}}{\ecmd'}{\cmd'}{\tau'}{\prio}$.
  By induction, $\cmdtyped[]{\esig}{\ctx}{\cmd}{\tau}{\prio}$ and
  $\cmdtyped[]{\esig}{\ctx, \hastype{x}{\tau}}{\cmd'}{\tau'}{\prio}$.
  Apply rules \rulename{\cmdsym I} and \rulename{Bind}.
\item By inversion, $\elabinst{\ctx}{\inst}{\cmd}{\tau}{\prio}$.
  By induction, $\cmdtyped[]{\esig}{\ctx}{\cmd}{\tau}{\prio}$.
  \end{itemize}
  \fi
\item By induction on the derivation of $\elabdecl{\ctx}{\decl}{x}{e}{\tau}$
  \begin{itemize}
  \item $\decl = \kwdval{x}{e}$.
    By inversion, $\elabexp{\ctx}{\eexp}{e}{\tau}$. By induction,
    $\etyped[]{\esig}{\ctx}{e}{\tau}$.
  \item $\decl = \kwdfun{f}{x_1 \dots x_n}{\eexp}$.
    By inversion, $\elabexp{\ctx, \hastype{f}{\tau_f}, \hastype{x_1}{\tau_1},
    \dots, \hastype{x_n}{\tau_n}}{\eexp}{e}{\tau}$.
    By induction, $\etyped[]{\esig}{\ctx, \hastype{f}{\tau_f}, \hastype{x_1}{\tau_1},
    \dots, \hastype{x_n}{\tau_n}}{e}{\tau}$.
    By $n$ applications of \rulename{\arrsym I}, we have
    $\etyped[]{\esig}{\ctx, \hastype{f}{\tau_f}}{\kwfun{x_1}{\dots \kwfun{x_n}{e}}}
    {\tau_f}$. Finally, apply rule \rulename{fix}.
  \item $\kwdwfun{f}{\vprio_1:\cons_1 \dots \vprio_n:\cons_n}
    {x_1 \dots x_m}{\eexp}$.
    By inversion,
    \[\elabexp{\ctx,
    \hastype{f}{\tau_f},
    \vprio_1 \isprio, \cons_1, \dots, \vprio_n \isprio, \cons_n,
    \hastype{x_1}{\tau_1}, \dots, \hastype{x_m}{\tau_m}}
    {\eexp}{e}{\tau}\]
    By induction, $\etyped[]{\esig}{\ctx,
    \hastype{f}{\tau_f},
    \vprio_1 \isprio, \cons_1, \dots, \vprio_n \isprio, \cons_n,
    \hastype{x_1}{\tau_1}, \dots, \hastype{x_m}{\tau_m}}
    {e}{\tau}$.
    By $m$ applications of \rulename{\arrsym I}, we have
    \[\etyped[]{\esig}{\ctx, \hastype{f}{\tau_f}, \vprio_1 \isprio, \cons_1, \dots,
      \vprio_n \isprio, \cons_n}
    {\kwfun{x_1}{\dots \kwfun{x_m}{e}}}{\tau_1 \arrsym \dots \arrsym \tau_m \arrsym \tau}\]
    By $n$ applications of \rulename{\fasym I}, we have
    $\etyped[]{\esig}{\ctx, \hastype{f}{\tau_f}}
    {\kwwlam{\vprio_1}{\cons_1}{\dots \kwwlam{\vprio_n}{\cons_n}
        {\kwfun{x_1}{\dots \kwfun{x_m}{e}}}}}{\tau_f}$.
    Finally, apply rule \rulename{fix}.
  \end{itemize}
\item By induction on the derivation of $\elabprog{\worlds}{\ctx}{\prog}{\cmd}{\worlds'}{\ctx'}$.
  \begin{itemize}
  \item $\prog = \kwdprio{\prioc}~\prog'$. By inversion,
    $\elabprog{\worlds \cup \{\prioc\}}{\ctx}{\prog'}{\cmd}
    {\worlds'}{\ctx}$. By induction,
    $\cmdtyped[\worlds \cup \worlds' \cup \{\prioc\}]{\esig}{\ctx}{\cmd}{\tau}{\bprio}$.
  \item $\prog = \kwdple{\prioc_1}{\prioc_2}~\prog'$. By inversion,
    $\elabprog{(\worlds \cup \{(\prioc_1, \prioc_2)\})}{\ctx}{\prog'}{\cmd}
    {\worlds'}{\ctx}$. By induction,
    $\cmdtyped[\worlds \cup \worlds' \cup \{(\prioc_1, \prioc_2)\}]{\esig}{\ctx}{\cmd}{\tau}{\bprio}$.
  \item $\prog = \decl~\prog'$. By inversion,
    $\elabdecl{\ctxify{\worlds}, \ctx}{\decl}{x}{e}{\tau'}$ and
    $\elabprog{\worlds}{\ctx, \hastype{x}{\tau'}}{\prog'}{\cmd}
    {\worlds'}{\ctx}$. By induction,
    $\etyped[]{\esig}{\ctxify{\worlds}, \ctx}{e}{\tau'}$ and
    $\cmdtyped[\worlds \cup \worlds']{\ctx, \hastype{x}{\tau'}}
    {\cmd}{\tau}{\bprio}$. By Lemma~\ref{lem:ctxify},
    $\etyped[\worlds]{\esig}{\ctx}{e}{\tau'}$
    By weakening,
    $\etyped[\worlds \cup \worlds']{\esig}{\ctx}{e}{\tau'}$
    Apply typing rules~\rulename{Ret}, \rulename{\cmdsym I} and \rulename{Bind}.
  \item $\prog = \kwmain{\ecmd}$. By inversion,
    $\elabcmd{\ctxify{\worlds}, \ctx}{\ecmd}{\cmd}{\tau}{\bprio}$.
    By induction,
    $\cmdtyped[]{\esig}{\ctxify{\worlds}, \ctx}{\cmd}{\tau}{\bprio}$.
    By Lemma~\ref{lem:ctxify},
    $\cmdtyped[\worlds]{\esig}{\ctx}{\cmd}{\tau}{\bprio}$.
  \end{itemize}
\end{enumerate}
\end{proof}

The main result is the correctness of the elaboration of an entire {\langname}
program in an empty context with only the priority~$\bot$ initially defined.
This is a simple application of the last part of Theorem~\ref{thm:elab-corr}.

\begin{cor}
  If $\elabprog{\{\bot\}}{\cdot}{\prog}{\cmd}{\worlds}{\ctx}$,
  then $\cmdtyped[\worlds \cup \{\bot\}]{\esig}{\cdot}{\cmd}{\tau}{\bprio}$.
\end{cor}


==> fig-elab.tex <==
\begin{figure}
\[
\begin{array}{llll}
  \mathit{Expressions} & \eexp & \bnfdef & x \bnfalt
  \kwtriv \bnfalt
  \kwn \bnfalt
  \kwifz{\eexp}{\eexp}{x}{\eexp} \bnfalt
  \kwfun{x}{\eexp} \bnfalt
  \kwapply{\eexp}{\eexp} \bnfalt
  \kwpair{\eexp}{\eexp} \bnfalt
  \kwfst{\eexp} \bnfalt
  \kwsnd{\eexp} \\ & & & \bnfalt
  \kwinl{\eexp} \bnfalt
  \kwinr{\eexp} \bnfalt
  \kwcase{\eexp}{x}{\eexp}{y}{\eexp} \bnfalt
  \kwoutput{\eexp} \bnfalt
  \kwinput \\ & & & \bnfalt
  \kwcmd{\prio}{\ecmd} \bnfalt
  \kwwlam{\vprio}{\cons}{\eexp} \bnfalt
  \kwwapp{\eexp}{\prio} \bnfalt
  \kwlet{\multi{\decl}}{\eexp}
  \\

  \mathit{Instructions} & \inst & \bnfdef & \kwdo{\eexp} \bnfalt
  \kwbspawn{\prio}{\tau}{\ecmd} \bnfalt
  \kwbsync{\eexp}\bnfalt
  \kwret{\eexp}
  %\eexp
  \\

  \mathit{Commands} & \ecmd & \bnfdef & \kwbind{\inst}{x}{\ecmd} \bnfalt
  \inst\\

  \mathit{Prio.~Annotations} & \priocons & \bnfdef & \vprio : \cons\\

  \mathit{Declarations} & \decl & \bnfdef & \kwdval{x}{\eexp} \bnfalt
  \kwdfun{f}{\multip{x}}{\eexp} \bnfalt
  \kwdwfun{f}{\multip{\priocons}}{\multip{x}}{\eexp}\\

  \mathit{Toplevel~Decls.} & \tdecl & \bnfdef & \decl \bnfalt
  \kwdprio{\prioc} \bnfalt
  \kwdplt{\prioc}{\prioc} %\bnfalt
  %\kwdplt{\prioc}{\prioc}
  \\

  \mathit{Programs} & \prog & \bnfdef & \kwmain{\ecmd} \bnfalt \tdecl~\prog\\
\end{array}
\]
\caption{Formal syntax of {\langname} for elaboration.}
\label{fig:elab-syn}
\end{figure}

\begin{figure}
  \[
  \begin{array}{c}
\ifproofs
\infer
{
\strut
}
{
\elabexp{\ctx}{\kwtriv}{\kwtriv}{\kwunit}
}

\qquad

\infer
{
\strut
}
{
\elabexp{\ctx}{\kwn}{\kwn}{\kwnat}
}

\\[4ex]

\infer
{
  \elabexp{\ctx}{\eexp}{e}{\kwnat}\\
  \elabexp{\ctx}{\eexp_1}{e_1}{\tau}\\
  \elabexp{\ctx,\hastype{x}{\kwnat}}{\eexp_2}{e_2}{\tau}
}
{
  \elabexp{\ctx}{\kwifz{\eexp}{\eexp_1}{x}{\eexp_2}}
          {\kwifz{e}{e_1}{x}{e_2}}{\tau}
}

\\[4ex]

\infer
{
  \elabexp{\ctx, \hastype{x}{\tau_1}}{\eexp}{e}{\tau_2}
}
{
  \elabexp{\ctx}{\kwfun{x}{\eexp}}{\kwfun{x}{e}}{\kwarr{\tau_1}{\tau_2}}
}

\qquad

\infer
{
\elabexp{\ctx}{\eexp_1}{e_1}{\kwarr{\tau_1}{\tau_2}}\\
\elabexp{\ctx}{\eexp_2}{e_2}{\tau_1}
}
{
\elabexp{\ctx}{\kwapply{\eexp_1}{\eexp_2}}{\kwapply{e_1}{e_2}}{\tau_2}
}

\\[4ex]

\infer
{
  \elabexp{\ctx}{\eexp_1}{e_1}{\tau_1}\\
  \elabexp{\ctx}{\eexp_2}{e_2}{\tau_2}
}
{
  \elabexp{\ctx}{\kwpair{\eexp_1}{\eexp_2}}
          {\kwpair{e_1}{e_2}}{\kwprod{\tau_1}{\tau_2}}
}

\\[4ex]

\infer
{
  \elabexp{\ctx}{\eexp}{e}{\kwprod{\tau_1}{\tau_2}}
}
{
  \elabexp{\ctx}{\kwfst{\eexp}}{\kwfst{e}}{\tau_1}
}

\qquad

\infer
{
  \elabexp{\ctx}{\eexp}{e}{\kwprod{\tau_1}{\tau_2}}
}
{
  \elabexp{\ctx}{\kwsnd{\eexp}}{\kwsnd{e}}{\tau_1}
}

\\[4ex]

\infer
{
  \elabexp{\ctx}{\eexp}{e}{\tau_1}
}
{
  \elabexp{\ctx}{\kwinl{\eexp}}{\kwinl{e}}{\kwsum{\tau_1}{\tau_2}}
}

\qquad

\infer
{
  \elabexp{\ctx}{\eexp}{e}{\tau_2}
}
{
  \elabexp{\ctx}{\kwinr{\eexp}}{\kwinr{e}}{\kwsum{\tau_1}{\tau_2}}
}

\\[4ex]

\infer
{
  \elabexp{\ctx}{\eexp}{e}{\kwsum{\tau_1}{\tau_2}}\\
  \elabexp{\ctx,\hastype{x}{\tau_1}}{\eexp_1}{e_1}{\tau'}\\
  \elabexp{\ctx,\hastype{y}{\tau_2}}{\eexp_2}{e_2}{\tau'}
}
{
  \elabexp{\ctx}{\kwcase{\eexp}{x}{\eexp_1}{y}{\eexp_2}}
          {\kwcase{e}{x}{e_1}{y}{e_2}}{\tau'}
}

\\[4ex]
\fi

\infer
{
  \elabexp{\ctx}{\eexp}{e}{\kwnat}
}
{
  \elabexp{\ctx}{\kwoutput{\eexp}}{\kwoutput{e}}{\kwunit}
}

\qquad

\infer
{
  \strut
}
{
  \elabexp{\ctx}{\kwinput}{\kwinput}{\kwnat}
}

\\[4ex]

\infer
{
  \elabcmd{\ctx}{\ecmd}{\cmd}{\tau}{\prio}
}
{
  \elabexp{\ctx}{\kwcmd{\prio}{\ecmd}}
          {\kwcmd{\prio}{\cmd}}{\kwcmdt{\tau}{\prio}}
}

\\[4ex]

\infer
{
  \elabexp{\ctx, \vprio \isprio, \cons}{\eexp}{e}{\tau}
}
{
  \elabexp{\ctx}{\kwwlam{\vprio}{\cons}{\eexp}}
          {\kwwlam{\vprio}{\cons}{e}}{\kwforall{\vprio}{\cons}{\tau}}
}

\qquad

\infer
{
  \elabexp{\ctx}{\eexp}{e}{\kwforall{\vprio}{\cons}{\tau}}\\
  \meetc[]{\ctx}{[\prio'/\vprio]\cons}
}
{
  \elabexp{\ctx}{\kwwapp{\eexp}{\prio'}}
          {\kwwapp{e}{\prio'}}
          {[\prio'/\vprio]\tau}
}

\\[4ex]

\infer
{
  \elabexp{\ctx}{\eexp}{e}{\tau}
}
{
  \elabexp{\ctx}{\kwlet{}{\eexp}}{e}{\tau}
}

\quad

\infer
{
  \elabdecl{\ctx}{\decl}{x}{e'}{\tau'}\\
  \elabexp{\ctx, \hastype{x}{\tau'}}{\kwlet{\multi{\decl}}{\eexp}}{e}{\tau}
}
{
  \elabexp{\ctx}{\kwlet{\decl~\multi{\decl}}{\eexp}}
          {\kwapply{(\kwfun{x}{e})}{e'}}{\tau}
}

  \end{array}
  \]
  \caption{Elaboration of expressions\ifproofs.\else (selected rules).\fi}
  \label{fig:elab-exp}
\end{figure}

\begin{figure}
  \[
  \begin{array}{c}
\infer
{
  \elabexp{\ctx}{\eexp}{e}{\kwcmdt{\tau}{\prio}}\\
  x \fresh
}
{
  \elabinst{\ctx}{\kwdo{\eexp}}{\kwbind{e}{x}{\kwret{x}}}{\tau}{\prio}
}

\qquad

\infer
{
  \elabexp{\ctx}{\eexp}{e}{\kwat{\tau}{\prio'}}\\
  \meetc[]{\ctx}{\ple{\prio}{\prio'}}\\
}
{
  \elabinst{\ctx}{\kwbsync{\eexp}}
           {\kwbsync{e}}
           {\tau}{\prio}
}

\\[4ex]

\infer
{
  \elabcmd{\ctx}{\ecmd}{\cmd}{\tau}{\prio'}
}
{
  \elabinst{\ctx}{\kwbspawn{\prio'}{\tau}{\ecmd}}
           {\kwbspawn{\prio'}{\tau}{\cmd}}
           {\kwat{\tau}{\prio'}}{\prio}
}

\\[4ex]

\infer
{
  \elabexp{\ctx}{\eexp}{e}{\tau}
}
{
  \elabinst{\ctx}{\kwret{\eexp}}
           {\kwret{e}}
           {\tau}{\prio}
}

\\[4ex]

\infer
{
  \elabinst{\ctx}{\inst}{\cmd}{\tau}{\prio}\\
  \elabcmd{\ctx, \hastype{x}{\tau}}{\ecmd'}{\cmd'}{\tau'}{\prio}
}
{
  \elabcmd{\ctx}{\kwbind{\inst}{x}{\ecmd'}}
          {\kwbind{\kwcmd{\prio}{\cmd}}{x}{\cmd'}}{\tau'}{\prio}
}

\qquad

\infer
{
  \elabinst{\ctx}{\inst}{\cmd}{\tau}{\prio}\\
}
{
  \elabcmd{\ctx}{\inst}{\cmd}{\tau}{\prio}
}
  \end{array}
  \]
  \caption{Elaboration of instructions and threads.}
  \label{fig:elab-thread}
\end{figure}

\begin{figure}
\[
\begin{array}{c}
\infer
{
  \elabexp{\ctx}{\eexp}{e}{\tau}
}
{
  \elabdecl{\ctx}{\kwdval{x}{\eexp}}{x}{e}{\tau}
}

\\[4ex]

\infer
{
  \tau_f = \kwarr{\tau_1}{\kwarr{\dots}{\kwarr{\tau_n}{\tau}}}\\
  \elabexp{\ctx, \hastype{f}{\tau_f},
    \hastype{x_1}{\tau_1}, \dots, \hastype{x_n}{\tau_n}}
          {\eexp}{e}{\tau}
}
{
  \elabdecl{\ctx}{\kwdfun{f}{x_1 \dots x_n}{\eexp}}{f}
           {\kwfix{f}{\tau_f}
             {\kwfun{x_1}{\dots \kwfun{x_n}{e}}}}
           {\tau_f}
}

\\[4ex]

\infer
{
  \tau_f = \kwforall{\vprio_1}{\cons_1}{\dots \kwforall{\vprio_n}{\cons_n}{
          \kwarr{\tau_1}{\kwarr{\dots}{\kwarr{\tau_m}{\tau}}}}}\\
  \elabexp{\ctx,
    \hastype{f}{\tau_f},
    \vprio_1 \isprio, \cons_1, \dots, \vprio_n \isprio, \cons_n,
    \hastype{x_1}{\tau_1}, \dots, \hastype{x_m}{\tau_m}}
          {\eexp}{e}{\tau}\\
          e_{\mathit{body}} =
            \kwwlam{\vprio_1}{\cons_1}{\dots \kwwlam{\vprio_n}{\cons_n}{
      \kwfun{x_1}{\dots \kwfun{x_m}{e}}}}
}
{
  \elabdecl{\ctx}{\kwdwfun{f}{\vprio_1:\cons_1 \dots \vprio_n:\cons_n}
    {x_1 \dots x_m}{\eexp}}{f}
           {\kwfix{f}{\tau_f}
             {e_\mathit{body}}}
           {\tau_f}
}

\\[4ex]

\infer
{
  \elabprog{\worlds \cup \{\prioc\}}{\ctx}{\prog}{\cmd}
             {\worlds'}{\ctx'}
}
{
  \elabprog{\worlds}{\ctx}{\kwdprio{\prioc}~\prog}
             {\cmd}{\worlds' \cup \{\prioc\}}{\ctx'}
}

\\[4ex]

\infer
{
  \prioc_1, \prioc_2 \in \worlds\\
  \nple{\prioc_2}{\prioc_1}\\
  \elabprog{(\worlds \cup \{(\prioc_1, \prioc_2)\})}{\ctx}
             {\prog}{\cmd}
             {\worlds'}{\ctx'}
}
{
  \elabprog{\worlds}{\ctx}{\kwdplt{\prioc_1}{\prioc_2}~\prog}
             {\cmd}{\worlds' \cup \{(\prioc_1, \prioc_2)\}}{\ctx'}
}

\\[4ex]

\infer
{
  \elabdecl{\ctxify{\worlds},\ctx}{\decl}{x}{e}{\tau}\\
  \elabprog{\worlds}{\ctx, \hastype{x}{\tau}}
             {\prog}{\cmd}{\worlds'}{\ctx'}
}
{
  \elabprog{\worlds}{\ctx}{\decl~\prog}
           {\kwbind{\kwcmd{\bprio}{\kwret{e}}}{x}{\cmd}}
           {\worlds'}{\ctx'}
}

\qquad

\infer
{
  \elabcmd{\ctxify{\worlds}, \ctx}{\ecmd}{\cmd}{\tau}{\bprio}
}
{
  \elabprog{\worlds}{\ctx}{\kwmain{\ecmd}}{\cmd}{\emptyset}{\ctx}
}
\end{array}
\]
\caption{Elaboration of declarations and programs.}
\label{fig:elab-prog}
\end{figure}

